Non-Interactive Symbolic-Aided Chain-of-Thought for Logical Reasoning

This work introduces Symbolic-Aided Chain-of-Thought (CoT), an improved approach to standard CoT, for logical reasoning in large language models (LLMs). The key idea is to integrate lightweight symbolic representations into few-shot prompts, structuring the inference steps with a consistent strategy to make reasoning patterns more explicit within a non-interactive reasoning process. By incorporating these symbolic structures, Symbolic-Aided CoT preserves the generalizability of standard prompting techniques while enhancing the transparency, interpretability, and analyzability of LLM logical reasoning. Extensive experiments on four well-known logical reasoning benchmarks -- ProofWriter, FOLIO, ProntoQA, and LogicalDeduction, which cover diverse reasoning tasks and scenarios -- demonstrate the effectiveness of the proposed approach, particularly in complex reasoning tasks that require navigating multiple constraints or rules. Notably, Symbolic-Aided CoT consistently improves LLMs' reasoning capabilities across various model sizes and significantly outperforms conventional CoT on three out of four datasets, ProofWriter, ProntoQA, and LogicalDeduction.

==> model_size_ab.tex <==
idx depth Standard CoT LogicCoT
1.7 1.7 49.67 53.33 58.17
4 4 52.00 57.5 74.33
8 8 60.0 57.83 78.67
14 14 46.5 62.67 77.00
32 32 52.33 72.17 79.17

==> model_size_ld.tex <==
idx depth Standard CoT LogicCoT
1.7 1.7 44.33 53.33 48.67
4 4 52.67 71.67 74.33
8 8 57.00 72.67 77.33
14 14 61.67 81.67 86.33
32 32 66.67 82.33 89.00 
